Proactive Provenance Policies for Automatic Cryptographic Data Centric Security

Data provenance analysis has been used as an assistive measure for ensuring system integrity. However, such techniques are typically reactive approaches to identify the root cause of an attack in its aftermath. This is in part due to fact that the collection of provenance metadata often results in a deluge of information that cannot easily be queried and analyzed in real time. This paper presents an approach for proactively reasoning about provenance metadata within the Automatic Cryptographic Data Centric (ACDC) security architecture, a new security infrastructure in which all data interactions are considered at a coarse granularity, similar to the Function as a Service model. At this scale, we have found that data interactions are manageable for the proactive specification and evaluation of provenance policies -- constraints placed on provenance metadata to prevent the consumption of untrusted data. This paper provides a model for proactively evaluating provenance metadata in the ACDC paradigm as well as a case study of an electronic voting scheme to demonstrate the applicability of ACDC and the provenance policies needed to ensure data integrity.

==> acdcarchPC.tex <==

\newcommand\todo[1]{\textcolor{red}{TODO: {#1}}}
\newcommand\tbd[1]{\textcolor{red}{TODO: {#1}}}
\newcommand\subsubsubsection[1]{{\bf #1}\par}
\newcommand\pterm[1]{{\tt#1}}



\section{The ACDC FaaS Paradigm}\label{sec:arch}
In order to support provenance collection at the necessary coarse granularity, we propose the Automatic Cryptographic Data-Centric Security (ACDC) model.


\begin{figure}[t]
\centering \includegraphics[width=.95\linewidth]{ACDCArch.jpg}
\caption{ACDC Core Component Architecture} \label{fig:arch}
\end{figure}

At its core, ACDC puts all data into encrypted secure data capsules (see Figure~\ref{fig:arch}). Each capsule contains cryptographically enforced access control policies that define who can access and use the data. Each capsule also contains its provenance in the ACDC system, allowing authorized parties to assess a capsule's integrity before acting upon it. To perform computations, data owners can cryptographically authorize functions to run on their data. ACDC uses contracts to define what functions can be executed and how results will be protected. 
The function execution itself is protected by secure computation techniques like multiparty computation (MPC), functional encryption, or secure enclave created by trusted hardware. Data owners have control over which technique is allowed to process their data, enabling trade-offs between security, functionality, and performance. ACDC seamlessly enables different data owners to securely collaborate and share their data with strict owner-controlled limitations.
Finally, ACDC uses content-centric networking (CCN)~\cite{Jacobson:2009:NNC:1658939.1658941} to route and transmit data capsules by their names rather than by addressing the systems that have the data. This enables capsules' cryptographic protections to protect data wherever they go on the network. CCN also improves data availability with in-network caching and efficient content distribution. The following section provides a brief overview of the components of ACDC.


\subsection{Component Architecture}\label{sec:arch_comp_arch}

An instance of an ACDC network (closed or Interned-wide) comprises a set of nodes (e.g., dedicated servers) each running ACDC software and potentially a set of supporting servers that provide data for specific ACDC functionality using unspecified (back-end) protocols (e.g., the blockchain orderers may be a set of pre-existing servers that are independent of ACDC, but required for an ACDC provenance service node).

Certain nodes, such as Capsule Storage and FaaS provide network interfaces. ACDC imposes a naming scheme on those interfaces. In general, ACDC does not define any new network interfaces. Where possible, ACDC will use third party ICN protocols (like Named Data Networking) and, as needed, using an ICN overlay on a standard TCP/IP network.

This section enumerates the ACDC components.


{\bf Nodes}

In general, all ACDC nodes use a common ACDC core library. The library itself makes no distinction based on the node type. Nonetheless, the overall design is easier to describe by assigning a set of logical roles:
\begin{itemize}
\item [Compute Node] performs some computation on secure data
\item [Service Node] implements some function or service in response to a request (e.g., FaaS)
\item [Data Source] creates a new capsule from raw data
\item [Data Sink] obtains raw data from a capsule
\item [Authority Node] provides security tokens (e.g., keys or certificates), either out of band (e.g., to issue a node with a secret key), or via ACDC (e.g., to obtain a public key certificate or an attribute key)
\item [Capsule Storage Node] stores, routes, forwards, etc.\ data capsules (e.g., an NDN router)
\item [Provenance Orderer] supports the validity of the provenance data
\item [Provenance Server] appends provenance data and/or validates a provenance policy
\end{itemize}

{\bf Capsule Data}

ACDC data is stored in named, secure capsules. All capsules have digital signatures for authenticity and integrity. Encryption of the capsule data is optional.

{\bf Capsule Storage}

ACDC stores data capsules persistently, allowing nodes to publish new capsules, fetch existing capsules, and delete capsules. All capsules are named according to an ACDC naming scheme.

{\bf Function as a Service (FaaS)}

FaaS allows nodes to perform (or serve) one or more functions in a query/response model. In general, FaaS is expected to use the same naming schemes as capsule storage, such that any request can be static (Capsule Storage) or dynamic (FaaS).

{\bf Secure Execution Environment}
ACDC provides environments for secure execution. Example environment may include secure enclaves (e.g., Intel SGX) or MPC.

{\bf Policy}

ACDC policies specify how data can be used. Policies specify criteria for permitting an entity access to data. Policies, in general, are in the form of a boolean combination of terms, where each term could represent a role, identity, or proof of taking an action (such as checking revocation). ACDC defines a provenance policy for checking policy. Proof of validating a provenance policy could be a term in a data policy.

{\bf Keys}

ACDC uses various cryptographic keys for authentication, integrity, confidentiality, and access control. Most nodes will have at least one PKC secret key and/or at least one ABE key (such as MAABE).

\subsection{Design Details}\label{sec:arch_design}

\subsubsection{Data Capsule}\label{sec:data_capsule}

ACDC Data Capsules protect data. Capsules are named for storage and retrieval. All capsules include a digital signature for integrity and authenticity. Signature validation requires a PKI certificate path from the signer to a trusted root certificate. PKI certificates may themselves be placed within capsules.




Capsules provide confidentiality by encrypting the data field. The capsule policy controls access to the data decryption key. ACDC supports public data by using a blank (or empty) policy. The capsule data is encrypted under an encryption key. The encryption key is wrapped as the Encrypted Key field. The policy describes the set of keys necessary to decrypt the encryption key (and in turn, the data). 

The signer field indicates the data capsule creator and helps identify the public key to validate the signature.
The digital signature is computed over the entire capsule excluding the signature field itself.

\subsubsection{Capsule Storage}\label{sec:capsule_storage}

The capsule storage component provides a mechanism for accessing data capsules. Data capsules can be published into the capsule storage component and fetched (retrieved) by their names. Similarly, an appropriately authorized user (specifics to be decided) can delete content from a locally published store.

ACDC uses hierarchical naming scheme for naming capsules. The name should be roughly compatible with common ICN systems like NDN.

Functions:
\begin{itemize}
\item publish( named\_capsule )
\item fetch( name )
\item remove( name, TBD\_authorization\_data )
\end{itemize}

Publish() writes a new capsule to data storage. Fetch() attempts to obtain a copy of the capsule from storage. If successful, fetch() responds with the capsule data. If the data is not available or the node lacks permission to decrypt the data, fetch() should return with an error.

\subsubsection{Functions (FaaS)}\label{sec:functions}

Similar to Capsule Storage, Function as a Service allows nodes to obtain data from the ACDC network. FaaS generates data dynamically based on a request URI. As with traditional FaaS in a cloud environment, requests share a common URI scheme and routing with that of the data capsule storage component.

\subsubsection{Policy}\label{sec:policy}

ACDC uses policies to specify permissions. Data policies in a data capsule, for example, specify the permissions for obtaining a decryption key. Data policies of this form is the boolean combination of attribute terms, such as an MAABE policy string. The policy string contains a set of attribute terms separated by the boolean operators ``AND'' and ``OR.'' Parentheses should be used for explicit order of operations. Each attribute term has an attribute label and its authority's name separated by a hash mark ({\tt '\#'}). For example, \pterm{admin\_user\#ll} would be given to administrative users within the LL domain.

ACDC uses other forms of policies, e.g., within a contract. For example, a provenance policy defines a set of rules for checking data provenance.

\subsubsection{Contract}\label{sec:contract}

Contracts give conditions limiting how nodes can operate on data capsules. These restrictions may:
\begin{itemize}
\item restrict computation to a particular function,
\item further restrict the argument position for a function,
\item restrict who can perform computation (via a computation policy)
\item require provenance checks (via a provenance policy, as detailed in the following sections)
\item require revocation checks (via a revocation policy)
\end{itemize}

All contracts are expected to provide an output policy, which gives a list of restrictions to impose on the output data. Each input argument may have its own output policy, in which case, the output policies must be composed, thereby accumulating all the restrictions from each output policy (combining duplicate or potentially overlapping restrictions).


When creating a capsule, the source node assigns some data policy to the capsule. For each attribute term in the policy, the term's authority determines the specific criteria for issuing attributes to individual nodes. A source node can include a contract in the policy by using a term that maps to the contract. For example, the naming scheme could reserve labels starting with the string {\tt contract\_} for contract terms. In such a case, a compute node trying to operate on the data would need to obtain an attribute for the contract from the contract term's authority, e.g., via FaaS. The authority then decides if and how to issue the associated attribute to the compute node.

The contract itself need not be public. In some scenarios it is reasonable to publish the contract in a data capsule (either encrypted or in plaintext) conforming to the ACDC contract fields. In other scenarios, it may be advantageous for the authority to handle the contract locally using an ad hoc format. In the latter case, the authority has more flexibility in supporting non-standard policies and/or for the authority to apply the provenance and/or revocation policies. In addition to the attribute (e.g., an encrypted attribute key), the response from the authority would need to convey contract fields, such as the output policy.

\subsubsection{Provenance}\label{sec:arch_provenance}
ACDC records the creation and use of data capsules through provenance. When publishing a data capsule, ACDC adds provenance information for that capsule, including any dependencies on how the data was derived. For example, the provenance record for the data capsule created via a computation will include dependencies on the input data capsules, the function, and the node performing the computation. The full provenance graph is stored in a distributed, truncation-resistant ledger (i.e. a private blockchain.)


\subsubsection{Node}\label{sec:arch_node}
ACDC is middleware running over a distributed set of nodes, each running a separate instance of the ACDC software. Different nodes take different roles:

\begin{itemize}
\item [General purpose node] creates data, consumes data, and/or performs computation.

\item [ABE authority node] issues attribute keys and publishes its public keys.

\item [PKI authority node] issues certificates. In general, ACDC assumes that nodes obtain certificates for their key pair out of band. PKI authorities are responsible for publishing the public key certificates for the keys in its domain along with its own CA certificate. PKI authorities are responsible for providing certificate revocation (e.g., via publishing a revocation list).

\item [ACDC provenance node] handles requests to append provenance records and to check provenance (e.g., via FaaS).

\item [Provenance orderer node] distinct from the ACDC provenance node, a set of orderer nodes ensure the validity of the provenance blockchain. The orderers communicate directly with the ACDC provenance node(s) using implementation-specific protocols (e.g., through a third-party blockchain implementation) and hence do not include the ACDC library.

\item [Capsule storage node] supports the distribution of capsules. In general, capsule storage nodes do not include the ACDC library, except at the edge where ACDC nodes interact with capsules.
\end{itemize}

\subsubsection{Intrinsic ACDC Functions}\label{sec:arch_intrinsic}
ACDC provides a set of intrinsic functions, as opposed to the application-specific set of functions that compute nodes execute on capsule data. The intrinsic functions provide basic functionality essential to ACDC. Where possible these functions operate using the ACDC FaaS paradigm.

\begin{itemize}
\item The get\_auth\_key() function allows an authorized node to obtain an attribute key for a specific attribute term. The request includes the name of the attribute. The authority for the attribute's domain processes the request. It obtains the identity of the caller from the request and, if authorized, replies with the attribute key encrypted under the caller's private PKI key. The reply includes optional parameters, such as a contract's output policy, if appropriate for the requested attribute.

\item The check\_provenance() function takes a provenance policy string and a hash value identifying a data capsule's provenance record, verifies the policy string against the provenance data, and returns the result (e.g., does the provenance for the data satisfy the policy).

\item The append\_provenance() function appends a provenance record for a new data capsule. The provenance record contains information about each of the data capsule's dependencies.
\end{itemize}




==> acdcarchPrecut.tex <==

\newcommand\todo[1]{\textcolor{red}{TODO: {#1}}}
\newcommand\tbd[1]{\textcolor{red}{TODO: {#1}}}
\newcommand\subsubsubsection[1]{{\bf #1}\par}
\newcommand\pterm[1]{{\tt#1}}



\section{The ACDC FaaS Paradigm}\label{sec:arch}
In order to support provenance collection at the necessary coarse granularity, we propose the Automatic Cryptographic Data-Centric Security (ACDC) model.


\begin{figure}[t]
\centering \includegraphics[width=.95\linewidth]{ACDCArch.jpg}
\caption{ACDC Core Component Architecture} \label{fig:arch}
\end{figure}

At its core, ACDC puts all data into encrypted secure data capsules (see Figure~\ref{fig:arch}). Each capsule contains cryptographically enforced access control policies that define who can access and use the data. Each capsule also contains its provenance in the ACDC system, allowing authorized parties to assess a capsule's integrity before acting upon it. To perform computations, data owners can cryptographically authorize functions to run on their data. ACDC uses contracts to define what functions can be executed and how results will be protected. 
The function execution itself is protected by secure computation techniques like multiparty computation (MPC), functional encryption, or secure enclave created by trusted hardware. Data owners have control over which technique is allowed to process their data, enabling trade-offs between security, functionality, and performance. ACDC seamlessly enables different data owners to securely collaborate and share their data with strict owner-controlled limitations.
Finally, ACDC uses content-centric networking (CCN)~\cite{Jacobson:2009:NNC:1658939.1658941} to route and transmit data capsules by their names rather than by addressing the systems that have the data. This enables capsules' cryptographic protections to protect data wherever they go on the network. CCN also improves data availability with in-network caching and efficient content distribution. The following section provides a brief overview of the components of ACDC.


\subsection{Component Architecture}\label{sec:arch_comp_arch}

An instance of an ACDC network (closed or Interned-wide) comprises a set of nodes (e.g., dedicated servers) each running ACDC software and potentially a set of supporting servers that provide data for specific ACDC functionality using unspecified (back-end) protocols.

Certain nodes, such as Capsule Storage and FaaS provide network interfaces. ACDC imposes a naming scheme on those interfaces. In general, ACDC does not define any new network interfaces. Where possible, ACDC will use third party ICN protocols (like Named Data Networking) and, as needed, using an ICN overlay on a standard TCP/IP network.

ACDC is constituted out of the following components.

{\bf Nodes}

In general, all ACDC nodes use a common ACDC core library. The library itself makes no distinction based on the node type. Nonetheless, the overall design is easier to describe by assigning a set of logical roles:
\begin{itemize}
\item [Compute Node] performs some computation on secure data
\item [Service Node] implements some function or service in response to a request (e.g., FaaS)
\item [Data Source] creates a new capsule from raw data
\item [Data Sink] obtains raw data from a capsule
\item [Authority Node] provides security tokens (e.g., keys or certificates), either out of band (e.g., to issue a node with a secret key), or via ACDC (e.g., to obtain a public key certificate or an attribute key)
\item [Capsule Storage Node] stores, routes, forwards, etc.\ data capsules (e.g., an NDN router)
\item [Provenance Orderer] supports the validity of the provenance data
\item [Provenance Server] appends provenance data and/or validates a provenance policy
\end{itemize}

{\bf Capsule Data}

ACDC data is stored in named, secure capsules. All capsules have digital signatures for authenticity and integrity. Encryption of the capsule data is optional.

{\bf Capsule Storage}

ACDC stores data capsules persistently, allowing nodes to publish new capsules, fetch existing capsules, and delete capsules. All capsules are named according to an ACDC naming scheme.

{\bf Function as a Service (FaaS)}

FaaS allows nodes to perform (or serve) one or more functions in a query/response model. In general, FaaS is expected to use the same naming schemes as capsule storage, such that any request can be static (Capsule Storage) or dynamic (FaaS).

{\bf Secure Execution Environment}
ACDC provides environments for secure execution. Example environment may include secure enclaves (e.g., Intel SGX) or MPC.

{\bf Policy}

ACDC policies specify how data can be used. Policies specify criteria for permitting an entity access to data. Policies, in general, are in the form of a boolean combination of terms, where each term could represent a role, identity, or proof of taking an action (such as checking revocation). ACDC defines a provenance policy for checking policy. Proof of validating a provenance policy could be a term in a data policy.

{\bf Keys}

ACDC uses various cryptographic keys for authentication, integrity, confidentiality, and access control. Most nodes will have at least one PKC secret key and/or at least one ABE key (such as MAABE).

\subsection{Design Details}\label{sec:arch_design}

\subsubsection{Data Capsule}\label{sec:data_capsule}

ACDC Data Capsules protect data. Capsules are named for storage and retrieval. All capsules include a digital signature for integrity and authenticity. Signature validation requires a PKI certificate path from the signer to a trusted root certificate. PKI certificates may themselves be placed within capsules.




Capsules provide confidentiality by encrypting the data field. The capsule policy controls access to the data decryption key. ACDC supports public data by using a blank (or empty) policy. The capsule data is encrypted under an encryption key. The encryption key is wrapped as the Encrypted Key field. The policy describes the set of keys necessary to decrypt the encryption key (and in turn, the data). 

The signer field indicates the data capsule creator and helps identify the public key to validate the signature.
The digital signature is computed over the entire capsule excluding the signature field itself.


\subsubsection{Policy}\label{sec:policy}

ACDC uses policies to specify permissions. Data policies in a data capsule, for example, specify the permissions for obtaining a decryption key. Data policies of this form is the boolean combination of attribute terms, such as an MAABE policy string. The policy string contains a set of attribute terms separated by the boolean operators ``AND'' and ``OR.'' Parentheses should be used for explicit order of operations. Each attribute term has an attribute label and its authority's name separated by a hash mark ({\tt '\#'}). For example, \pterm{admin\_user\#ll} would be given to administrative users within the LL domain.

ACDC uses other forms of policies, e.g., within a contract. For example, a provenance policy defines a set of rules for checking data provenance.

\subsubsection{Contract}\label{sec:contract}

Contracts give conditions limiting how nodes can operate on data capsules. These restrictions may:
\begin{itemize}
\item restrict computation to a particular function,
\item further restrict the argument position for a function,
\item restrict who can perform computation (via a computation policy)
\item require provenance checks (via a provenance policy, as detailed in the following sections)
\item require revocation checks (via a revocation policy)
\end{itemize}

All contracts are expected to provide an output policy, which gives a list of restrictions to impose on the output data. Each input argument may have its own output policy, in which case, the output policies must be composed, thereby accumulating all the restrictions from each output policy (combining duplicate or potentially overlapping restrictions).


When creating a capsule, the source node assigns some data policy to the capsule. For each attribute term in the policy, the term's authority determines the specific criteria for issuing attributes to individual nodes. A source node can include a contract in the policy by using a term that maps to the contract. For example, the naming scheme could reserve labels starting with the string {\tt contract\_} for contract terms. In such a case, a compute node trying to operate on the data would need to obtain an attribute for the contract from the contract term's authority, e.g., via FaaS. The authority then decides if and how to issue the associated attribute to the compute node.

The contract itself need not be public. In some scenarios it is reasonable to publish the contract in a data capsule (either encrypted or in plaintext) conforming to the ACDC contract fields. In other scenarios, it may be advantageous for the authority to handle the contract locally using an ad hoc format. In the latter case, the authority has more flexibility in supporting non-standard policies and/or for the authority to apply the provenance and/or revocation policies. In addition to the attribute (e.g., an encrypted attribute key), the response from the authority would need to convey contract fields, such as the output policy.

\subsubsection{Node}\label{sec:arch_node}
ACDC is middleware running over a distributed set of nodes, each running a separate instance of the ACDC software.


==> fw.tex <==
\section{Future Work}\label{sec:fw}
There are two primary directions for future work stemming from this initial policy design and evaluation.

First, and foremost, is the expansion of the ACDC framework. Securing data as a first-class citizen is an approach that has a myriad of benefits. 

Seondly, there is independent advancement of  provenance policies in the Function as a Service (FaaS) execution model. Such an expansion could enable clients of services such as AWS lambda to untangle the currently inscrutiable chain of custody for inputs and products used in FaaS-style exection. This will entail the introduction of a distributed truncation-resistance store and provenance hooks into FaaS job specifications, but could be handeled entirely on the clients' end.

==> related_work.tex <==
\section{Related Work}

Several frameworks proposed for analyzing provenance metadata do so reactively and in retrospect, relying on either human analysis or the use of automated tools that may rely on machine learning techniques to characterize provenance graphs. Reactive security has benefits in areas such as identifying the root cause of an attack~\cite{lee2013high} and security auditing to ensure compliance with company policies~\cite{pasquier2018data}. While useful, these security practices do not actively prevent security mishaps. Proactive security practices should also be used in conjunction with reactive security practices. However, when security policies are specified proactively, with the intent of being enforced, they must be reasoned about in a precise and unambiguous way. Relevant to this work is proactive security policy specification to reason about provenance metadata, which has received little attention in the literature. 

Much work related to data provenance has focused in the areas of provenance collection (e.g.,~\cite{imran2018aggregated,liang2017provchain,liang2017towards,tsai2007new,muniswamy2006provenance,muniswamy2010provenance,gehani2012spade,pohly2012hi}) and secure storage of provenance metadata (e.g.,~\cite{liang2017provchain,liang2017towards,michlmayr2009service,bates2013towards,braun2008securing,bates2015trustworthy}) . While both of these areas are foundational to provenance-aware systems, the usefulness of provenance metadata, in the context of security, comes in the ability to analyze such data to gain insight into and improve a computing environment's overall security posture. 

Due to the large amounts of data that provenance collection systems can capture, relying on human analysis is impractical and error prone~\cite{hassan2018towards}. Automated tools aim to simplify and make the analysis of provenance metadata more efficient; however, many tools in the literature do so at a loss in precision. Huynh et al.~\cite{huynh2018provenance} present an automated analysis technique that relies on network analysis and machine learning techniques, it is shown that their analysis technique is able to classify provenance graphs into predetermined categories with high accuracy. Han et al. present FRAPpuccino~\cite{han2017frappuccino}, a provenance-based intrusion detection framework that aims to distinguish benign from anomalous behavior using a machine learning approach. Although machine learning techniques improve the efficiency with which provenance graphs can be analyzed, in high security contexts, machine-learning based characterization of provenance graphs suffer in 2 ways: (1) the categories that provenance graphs can be classified as do not provide well-defined properties of the graphs and (2) the classification categories cannot provide formal guarantees about data due to the possibility of false positives and false negatives.

Pasquier et al.~\cite{pasquier2018runtime} present CamQuery, a framework for the runtime analysis of whole system provenance. Because analysis takes place at runtime, the framework takes a proactive approach to policy specification over provenance metadata by expressing policies in a programmable graph processing framework inspired by GraphChi~\cite{kyrola2012graphchi} and GraphX~\cite{gonzalez2014graphx}. Our approach differs from Pasquier et al. in that we present a formal approach to reason about provenance policies rather than presenting an implementation. We present a foundational approach to reason about policies expressed over data provenance based on a mathematical semantics of provenance graphs.

Lemay et al.~\cite{lemay2017automated} present a framework for automated analysis of provenance by using graph grammars as a way to characterize provenance graphs. However, because the class of graphs parseable by such grammar is restricted to regular grammars, precision is lost and some graphs become parseable that the analyst may not intend to be; therefore, this approach is not amenable to security policy specification in which the policy must be precise and unambiguous. 

Park et al.~\cite{park2012provenance}, present a model for provenance-based access control in which policies are specified using propositional logic as an underlying formalism. This proactive approach to policy specification can provide formal guarantees about the data whose provenance conforms to the policy. Our approach differs from Park et al.'s domain specific approach in that we aim to provide a more general and expressive framework for provenance policy specification by using predicate logic as an underlying formalism. 


